Kairos: Practical Intrusion Detection and Investigation using Whole-system Provenance

Provenance graphs are structured audit logs that describe the history of a system's execution. Recent studies have explored a variety of techniques to analyze provenance graphs for automated host intrusion detection, focusing particularly on advanced persistent threats. Sifting through their design documents, we identify four common dimensions that drive the development of provenance-based intrusion detection systems (PIDSes): scope (can PIDSes detect modern attacks that infiltrate across application boundaries?), attack agnosticity (can PIDSes detect novel attacks without a priori knowledge of attack characteristics?), timeliness (can PIDSes efficiently monitor host systems as they run?), and attack reconstruction (can PIDSes distill attack activity from large provenance graphs so that sysadmins can easily understand and quickly respond to system intrusion?). We present KAIROS, the first PIDS that simultaneously satisfies the desiderata in all four dimensions, whereas existing approaches sacrifice at least one and struggle to achieve comparable detection performance. Kairos leverages a novel graph neural network-based encoder-decoder architecture that learns the temporal evolution of a provenance graph's structural changes to quantify the degree of anomalousness for each system event. Then, based on this fine-grained information, Kairos reconstructs attack footprints, generating compact summary graphs that accurately describe malicious activity over a stream of system audit logs. Using state-of-the-art benchmark datasets, we demonstrate that Kairos outperforms previous approaches.

==> __latexindent_temp.tex <==
\subsection{Framework Overview}
To preserve the features of dynamic behaviors in the host logs, the logs are processed into provenance graphs. To further exploit the features of nodes, the provenance graphs are processed into temporal graphs to preserve the causal relationships between behaviors as well as the features of nodes. The spatio-temporal characteristics of the graph can reflect the causal relationships between behaviors. Then, the structural and temporal features in the spatio-temporal graph are extracted via dynamic graph representation learning methods. Finally, anomalous behavior is detected by the anomaly detection module and the anomaly detection results are analyzed for interpretability with the help of additional information output by the representation learning method.

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/Kairos-architecture.eps}
  \caption{Kairos Architecture Overview. \notetp{This needs to be redone to help readers better understand what is going on.}\notetp{I suggest renaming the graph feature vector or whatever as edge list. Also do we collect from several machines in a single graph? If not just remove the two comptuers.}}
  \label{fig:arch}
\end{figure*}

\notetp{add a paragraph transitioning from the background section that set the stage for the problem we are solving.}
We give an overview of Kairos architecture in \autoref{fig:arch}.

\noindgras{\circled{1} Building Temporal Graph.} \notetp{briefly explain what it does.}

\noindgras{\circled{2} Representation Learning.} \notetp{briefly explain what it does.}

\noindgras{\circled{3} Anomaly Detection.} \notetp{briefly explain what it does.}

\noindgras{\circled{4} Anomaly Investigation.} \notetp{briefly explain what it does.}

\subsection{Data Collection and Representation}
\label{sec:framework:building}

\notezj{Following is the bullet point.}

\system's data source is the host kernel-level logs, which record any traces of behavior left behind. The components for log collection are Camflow\cite{camflow:pasquier:2017}, ETW\cite{etw}, etc. They can all reflect the operation relationship between subject and object by capturing each event log, and the raw log can be formally expressed as $<subject, operation, object, timestamp>$ after processing. This formal representation is a common format for provenance graphs.

In order to extract the features of the nodes for learning by the representation learning model, the traceability graph needs to be processed into a Temporal Graph. In the temporal graph, each edge is described as an operation performed on the destination node by the source node. After adding the features of the node, the format of the edge becomes: $<src\_node\_feature\_vec, edge\_feature\_vec,\\ dst\_node\_feature\_vec>$. Where node feature vec is generated from the features of the node after embedding. A good node embedding method should satisfy three conditions: 1. vector representations of nodes with similar roles are closer together in vector space; 2. able to handle unseen nodes; and 3. as simple as possible, since the embedded vectors will also be trained by the downstream model. Therefore, we use a hierarchical hash approach\cite{zhang2020dynamic   } to embed the path name of process and file nodes, IP address in socket nodes into vector space. Finally, all the host logs are processed into a temporal graph. The temporal graph consists of four parts: 1) source node set, 2) destination node set, 3) edge feature vector, 4) timestamp of edge happened.



\notetp{Discuss why we need to build a feature vector and the constraint we have without copying the SIGL paper. Discuss also why we represent the system execution as a graph (unless it was done earlier in the paper).}


\system learns the temporal and structural features of a provenance graph
from individual edges \notetp{the structurl and temporal aspect is the next subsection. Here it is about taking system logs and building a streaming provenance graph as an edge list.}
that describe various interactions (\ie dependency relationships)
between kernel objects,
which are represented by nodes.
\system considers three types of kernel objects
and 18 types of dependency relationships, as shown in~\autoref{}.
\system encodes the initial feature of a node
using a hierarchical feature hashing technique~\cite{zhang2020dynamic}
based on the type of the kernel object that the node represents.
Specifically,
\system uses the pathname
(and the pathname of the corresponding executable file)
as the initial feature of a file (and a process) node.
For socket nodes,
\system uses the destination IP addresses.
Pathnames and IP addresses are inherently hierarchical.
Hierarchical feature hashing~\cite{zhang2020dynamic} captures such information
while...




\subsection{Temporal and Structural Learning}
\label{sec:framework:learning}

The feature vectors we have generated at this point do not account for the graph structure and do not consider wider context surrounding individual events.
Applying an anomaly detection algorithm (\eg auto-encoder) over such embedding would be equivalent to past system call-based intrusion detection systems \notetp{cite a bunch of syscall-based techniques}.
However, \notetp{a sentence about why provenance/graph based techniques are superior.}
To address this issue we leverage the Temporal Graph Network (TGN) approach~\cite{rossi2020temporal} to build, through a streaming graph, per-event feature vectors that embed the full context surrounding each event.s

\notetp{Explain how the TGN works, what is the output \etc.}
The edge feature vectors we have generated in temporal graph do not account for the graph structure and do not consider wider context surrounding individual events. The causal relationships between all behaviors are preserved by the temporal graph and the attacks are causally linked in the graph.
Most of the existing methods transform the dynamic graph into a static graph and then extract the contextual information by using static graph analysis. This means that the integrity of the streaming graph is broken and the spatio-temporal features between behaviors are discarded.
To address this issue we leverage the Temporal Graph Network (TGN) approach~\cite{rossi2020temporal} to build, through history events in a streaming graph, per-node feature vectors that embed the full context of each nodes.
TGN uses history neighbor module to store history events associated with each node. Node memory module is used to track and store changes in the embedded features of the nodes. Based on memory module, TGN has ability to memorize long term dependencies for each node in temporal graph. Whenever a new event occurs, the history neighbor modules and node memory modules of the source and destination nodes involved are updated on the basis of the historical context.

\notezj{TODO: Explain the process of how to transform inputs to outputs.}

\textbf{The TGN input:} each event(edge) in temporal graph, the format is:
<source node, destination node, edge feature, edge timestamp>.

\textbf{The TGN output:} embedding vectors for each node involved in event streaming.

Core idea of TGN: predict the events that will occur in the next phase based on the events that have already occurred.

When \system receives event stream as input, it converts event stream into event batches in order to process it faster. Each event batch can be decomposed into a node set and an edge set. Then, the neighbor nodes corresponding to the history of the node are taken out according to the contents of the node set to get the structural information of the node history context. Get the historical feature embedding vector of the corresponding node from the node memory module.


\subsection{Negative Graphs}

\notetp{In its own subsection or in the anomaly detection part, we need to explain the negtive graph concept. Why do we need them? How do we build them? \etc}

\notezj{
  During the training phase, the model needs to learn behavioral patterns from benign behavioral data. Since the decoder is composed of linked predictor modules based on classifiers, the data used for training should contain 50\% benign samples and 50\% anomaly samples. Where the benign samples consists entirely of observed events. 

  The negative graph 
}


\subsection{Anomaly Detection}
\label{sec:framework:detection}

\notetp{We now have an embeding that represent the temporal and structural characteristic of our graph for each individual edges corresponding to a system event. We ingest those and do something clever to detect anomaly.}

\notezj{
  The TGN outputs are node embedding vectors, not events embedding vectors. But the decoder will calculate each event reconstruct loss based on the embedding vector of source node and destination node.

  The anomaly detection module will triger an alarm when
}

\subsection{Anomaly Reconstruction}
\label{sec:framework:investigation}

\notetp{We do not simply spit out a list of anomalous events, we reconstruct anomalous subgraphs that represent the attack.

  Explain how this work.

  Give an example with the ground truth description (as provided by DARPA or something) and show the corresponding subgraph.}


\subsection{Learning from False Positive}

\notetp{Can we feedback false positive into the training? Does it reduce their number if we do so? Can we evaluate this?}

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/pipeline.png}
  \caption{\notetp{The pipeline as I understand it at this point in time (2021-12-14). I took some inspirtion from the Holmes~\cite{holmes:milajerdi:2019} figure. It would be nice to iterate over that to converge towards something that aligns well with the text.}}
  \label{fig:pipeline}
\end{figure*}

==> add-intro.tex <==
This document %
contain materials supplementary 
to our paper published in 
the $43^{rd}$ IEEE Symposium on
Security and Privacy
(S\&P'24)~\cite{cheng2024kairos}.
In Section~\ref{sec:appendix:usecase}
of this document,
we report attack descriptions
based on the ground truth information
provided by the 
Defense Advanced Research Projects Agency
(DARPA)~\cite{darpa-e3,darpa-e5,darpa-optc}
and the associated attack summary graphs 
generated by \system.
In Section~\ref{sec:appendix:candidates},
we report representative false positive samples.


==> availability.tex <==
\system's code is available online
at \url{https://github.com/ProvenanceAnalytics/kairos}.
StreamSpot's~\cite{Manzoor2016FastMA} code and 
its datasets are available online
at \url{https://sbustreamspot.github.io/}.
Unicorn's~\cite{unicorn:han:2020} code is available online
at \url{https://github.com/crimson-unicorn}.
ThreaTrace's~\cite{wang2022threatrace} code is available online
at \url{https://github.com/threaTrace-detector/threaTrace}.
DARPA E3 and E5 datasets are available online
at \url{https://github.com/darpa-i2o/Transparent-Computing}.
DARPA OpTC datasets are available online
at \url{https://github.com/FiveDirections/OpTC-data}.


==> candidates.tex <==
\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_cadet3.png}
	\caption{A benign summary graph in DARPA's E3-CADETS dataset.}
	\label{fig:evaluation:casestudy_benign_cadets3}
\end{figure}

\noindgras{E3-CADETS (\autoref{fig:evaluation:casestudy_benign_cadets3}).}
\texttt{wget} is a Linux utility
used to download files from the Internet.
It might connect to any external IP or URL.
To determine
whether \texttt{wget}'s behavior
is related to attack activity,
sysadmins might either
check whether any connected IP
is in a blocklist
or confirm with the user
the identities of the files
they download.
Any file not recognized by the user
might be downloaded
by the attacker
through a C\&C server.

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_clearscope3.png}
	\caption{A benign summary graph in DARPA's E3-ClearScope.}
	\label{fig:evaluation:casestudy_benign_clearscope3}
\end{figure}

\noindgras{E3-ClearScope (\autoref{fig:evaluation:casestudy_benign_clearscope3}).}
\texttt{system\_server} is an Android core process
used to serve various Android system services,
\eg activity manager service (AMS).
Sysadmins can manually identify
whether a new legitimate system service
triggered \system' intrusion alert.

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_theia5.png}
	\caption{A benign summary graph in DARPA's E5-THEIA dataset.}
	\label{fig:evaluation:casestudy_benign_theia5}
\end{figure}

\noindgras{E5-THEIA (\autoref{fig:evaluation:casestudy_benign_theia5}).}
\texttt{dbus-daemon} provides one-to-one communication
between two applications\remove{in a system}.
\texttt{upowerd} is a Linux middleware
for power management,
which provides its services
\remove{(\eg notify status changes of power sources)}%
\remove{to applications}through \texttt{dbus}.
Sysadmins can check whether any application
using \texttt{dbus-daemon} \remove{for communication}%
is suspicious.

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_cadet5.png}
	\caption{A benign summary graph in DARPA's E5-CADETS dataset.}
	\label{fig:evaluation:casestudy_benign_cadets5}
\end{figure}

\noindgras{E5-CADETS (\autoref{fig:evaluation:casestudy_benign_cadets5}).}
\texttt{scp} is used to securely copy
files \remove{or folders }between Linux systems.
Unlike \texttt{wget}, %
it serves point-to-point file transfers,
\remove{meaning that}\change{so}
the user should know
the identity of the other host.
\texttt{du} is a Linux utility %
\remove{used to }\change{that} collects
a host's disk usage. %
Sysadmins could determine the legitimacy
of \texttt{scp} and \texttt{du} %
by checking
\remove{with the user}%
\remove{whether they are the one}%
\remove{who issues the commands.}%
\change{if the user issued
the commands.}

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_clearscope5.png}
	\caption{A benign summary graph in DARPA's E5-ClearScope.}
	\label{fig:evaluation:casestudy_benign_clearscope5}
\end{figure}

\noindgras{E5-ClearScope (\autoref{fig:evaluation:casestudy_benign_clearscope5}).}
\texttt{defcontainer} is a system process
associated with APK file installation.
Sysadmins might confirm with the user
the identities of the APK files
they install.
Sysadmins should further inspect
the installed APK files
to ensure that they are from legitimate vendors.

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/benign_optc.png}
	\caption{A benign summary graph in DARPA's OpTC.}
	\label{fig:evaluation:casestudy_benign_optc}
\end{figure}

\noindgras{OpTC (\autoref{fig:evaluation:casestudy_benign_optc}).}
\texttt{Installagent} is
Microsoft Windows Store's update agent,
which uses
the system services
\texttt{System}, \texttt{backgroundTaskHost}, and \texttt{svchost}.
Sysadmins need to investigate \texttt{Installagent}
only when suspicious files (\eg files not in the system path)
appear in its activity.




==> dimension-table.tex <==
\autoref{sec:background:summary-table}
summarizes recent PIDSes
along four dimensions.
Naturally, 
we do not include systems
that are not provenance-based
(\eg~\cite{DBLP:conf/ccs/LiuWZJXM19, DBLP:conf/ccs/Du0ZS17})
or do not perform intrusion detection
(\eg~\cite{han2021deepaid, sleuth:hossain:2017, priotracker:liu:2018, backtracking:king:2003, nodoze:hassan:2019}).

\begin{table}[t]
\caption{Summary of existing PIDSes along four dimensions (\autoref{sec:introduction}).
A system receives a \checkc \space if it (1) performs process- or application-specific analysis (\emph{scope});
(2) requires attack signatures and/or signals (\emph{attack agnosticity});
(3) analyzes offline or requires a full provenance graph to analyze (\emph{timeliness});
and/or (4) cannot reconstruct subgraphs of attack activity (\emph{attack reconstruction}).}
    \label{sec:background:summary-table}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|l|c|c|c|c|c|}
			\hline
			\textbf{System} & \textbf{Venue} & \textbf{Scope} &
			\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attack\\      Agnosticity\end{tabular}}}
			& \textbf{Timeliness} & 
			\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attack\\      Reconstruction\end{tabular}}} \\
			\hline
			StreamSpot~\cite{Manzoor2016FastMA} & KDD'16 & \checkm & \checkm & \checkm & \checkc \\ %
			Winnower~\cite{winnower:hassan:2018} & NDSS'18 & \checkc & \checkm & \checkm & \checkm \\ %
			Poirot~\cite{poirot:milajerdi:2019} & CCS'19 & \checkm & \checkc & \checkc & \checkm \\ %
			Holmes~\cite{holmes:milajerdi:2019} & S\&P'19 & \checkm & \checkc & \checkm & \checkm\\ %
			ProvDetector~\cite{provdetector:wang:2020} & NDSS'20 & \checkc & \checkm & \checkm & \checkc \\ %
			Unicorn~\cite{unicorn:han:2020} & NDSS'20 & \checkm & \checkm & \checkm & \checkc \\ %
			RapSheet~\cite{rapsheet:hassan:2020} & S\&P'20 & \checkm & \checkc & \checkc & \checkm \\ %
			SIGL~\cite{sigl:han:2021} & Security'21 & \checkc & \checkm & \checkc & \checkc \\ %
			Atlas~\cite{alsaheel2021atlas} & Security'21 & \checkm & \checkc & \checkm & \checkm \\ %
			Watson~\cite{zeng2021watson} & NDSS'21 & \checkm & \checkm & \checkc & \checkm \\ %
			ShadeWatcher~\cite{zengy2022shadewatcher} & S\&P'22 & \checkm & \checkm & \checkm & \checkc \\ %
			ThreaTrace~\cite{wang2022threatrace} & TIFS'22 & \checkm & \checkm & \checkm & \checkc \\ %
			\system & N/A & \checkm & \checkm & \checkm & \checkm\\
			\hline
	    \end{tabular}
    }
\end{table}


==> implementation.tex <==
\notetp{I wonder if we could have a shorter version of this in an availability statement (assuming we open-source everything).}
\notezj{In fact, I can't make the source code fully public. Parts of the copyrights owned by our institute will be used for other purposes later.
If Micheal and Thomas need the code, I can share it with you in private.
}

We prototype \system in \textcolor{red}{xxxK} lines of Python code.
We implement the hierarchical hash function(\autoref{sec:framework:building})
by using \emph{FeatureHasher} of Scikit-learn~\cite{sklearn}.
We use a relation database (PostgreSQL~\cite{postsql}) 
to store the processed provenance graphs 
which are collected from Windows, Linux and Android. 
\notetp{The DB part doesn't look like runtime detection.}
\notezj{The DB part is associated with our data preprocessing stage.}
We store the attributes and unique identification of nodes 
in different tables 
according to the node type.
The relationships between nodes are store in another \emph{event} table in triples.

Pytorch Geometric(PyG)\cite{Fey/Lenssen/2019} 
which uses PyTorch as backend 
is a library to train Graph Neural Networks (GNNs) 
for structured graph data. 
We use PyG to build the provenance graph learning module of \system. 
NetworkX\cite{hagberg2008exploring} is a Python library for studying complex graphs.
We use NetworkX to analyze 
the output of representation learning introduced in \autoref{sec:framework:learning}, 
\eg repeated edge merging, community detection.
Finally, we use GraphViz\cite{ellson2001graphviz} to visualize the result of investigation module.





==> meta_review.tex <==
\subsection*{Summary}
This paper presents \system, 
a provenance-based intrusion detection system.
\system applies GNN to analyze temporal information, 
which allows \system to capture attack behaviors 
that deviate from benign behaviors. 
In addition, the authors design an attack investigation method 
that analyzes sub-graphs denoting critical steps of attacks. 
The experiments show that \system outperforms existing methods.

\subsection*{Scientific Contributions}

\begin{itemize}
    \item Creates a New Tool to Enable Future Science
    \item Addresses a Long-Known Issue
\end{itemize}

\subsection*{Reasons for Acceptance}

\begin{enumerate}

\item \system uses a hierarchical feature extraction technique 
that enhances the overall detection capability. 
The system combines community detection algorithms and methods 
to identify rare nodes in the provenance graph, 
providing accurate detection.

\item This research addresses a critical and timely issue 
in the domain of APT detection.

\item The datasets and source code will be open source.

\end{enumerate}

\subsection*{Noteworthy Concerns}

\begin{enumerate}
\item The authors have successfully utilized GNNs for threat detection. 
However, several reviewers are concerned about the black-box nature of GNN. 
The lack of model explainability might hinder the adoption 
of the proposed system by incident responders 
while investigating threat alerts. 
By explaining how the alerts were generated by GNN 
can improve the adaptability of the proposed system.

\item Attackers continually develop new evasive techniques 
to bypass detection systems. 
There is a lack of detailed discussion on how the proposed system 
would adapt to such evolving threats. 
A more robust evaluation, 
considering adaptive attackers, 
would strengthen the paper's contributions.

\item While the paper presents impressive detection rates, 
there is less emphasis on the system's false positive rates. 
In practical scenarios,
a high number of false positives can lead to "alert fatigue" 
and undermine the effectiveness of the system.

\item Several reviewers have raised the concern related to concept drift. 
If the model is not updated frequently and adequately, 
it may fail to detect novel or evolved threats effectively. 
This lack of adaptability could severely limit the practical usefulness of the system. 
The paper should place a stronger emphasis on addressing concept drift, 
potentially by integrating continual learning strategies 
that would allow the model to evolve along with the threat landscape. 
The paper should also discuss the potential risk of data poisoning 
due to frequent retraining.

\end{enumerate}

==> response.tex <==
We thank IEEE S\&P 2023 and 2024 reviewers for their insightful questions. Our responses to their four concerns are:

\noindent\textbf{GNN's blackbox nature}:
While the GNN model \system uses is opaque, \system itself is not. 
The concise summary graphs \system generates from opaque GNN outputs
(\autoref{sec:framework:investigation}) 
provide actionable insights incident responders typically would need 
to investigate alerts. 
Combining interpretable ML techniques (e.g.,~\cite{han2021deepaid}) 
with \system will improve transparency but is orthogonal to this work.

\noindent\textbf{Evasion}: 
The existing techniques to evade provenance-based detectors are brute force, 
requiring almost full knowledge of the victim~\cite{goyalsometimes}. 
We evaluated \system using the published evasion dataset
to the best of our ability in~\autoref{sec:discussion}.
Given the lack of research in this area, 
we believe that sufficiently demonstrating robustness is complex enough 
to require a separate paper to address fully.

\noindent\textbf{False positive (FP)}: \system reports similar or lower FP rates 
compared to prior work, 
and we discuss in detail the causes of FPs in~\autoref{sec:evaluation:detection}. 
Anomaly-based detectors like \system 
trade off FP rates for the ability to detect unknown threats.

\noindent\textbf{Concept drift}: For an anomaly-based detector, 
evolving threats do not affect its model performance 
unless they become identical to the learned benign activity; 
this is similar to the evasion problem above. 
Evolving benign behavior, 
on the other hand, 
requires approaches like continuous learning to address. 
While our re-training strategy (\autoref{sec:evaluation:detection}) is primitive 
(albeit effective), 
it shows that \system is compatible with the latest study~\cite{DBLP:conf/ndss/HanWCW0W0WJ0SY23}, 
which performs selective re-training to combat concept drift, 
specifically in learning-based anomaly detection systems. 
We note that properly evaluating concept drift 
requires careful construction of provenance datasets; 
no such datasets are publicly available. 
While this is an important area for future work, 
it is well beyond the scope of this paper.

\emph{We direct readers to~\autoref{sec:discussion}, 
where the limitations of our work are fully discussed.}


==> use_cases.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=\textwidth, scale=0.5]{figures/case_study.png}
	\caption{A provenance summary graph from DARPA E3-THEIA that describes attack activity in the motivating example, as automatically generated by \system.
		Rectangles, ovals, and diamonds represent processes, files, and sockets, respectively.
		R=Read, W=Write, O=Open, S=Send, Rc=Receive, C=Clone, and E=Execute.
		We add colors and dashed elements for clarity 
		to highlight the output that \system generates.
		Solid nodes and edges are extracted by \system
		from the original provenance graph to \change{reconstruct the attack}.
		Dashed pink nodes and edges are attack-related activities missed by \system,
		according to the attack ground truth.
		Blue nodes and edges are activities not explicitly mentioned in the ground truth
		but included by \system.
	}
	\label{fig:motivation:e3theia-gt}
\end{figure*}

\noindgras{E3-THEIA (\autoref{fig:motivation:e3theia-gt}).} The attacker leverages a \texttt{Firefox} vulnerability
to establish a foothold on a victim machine,
which enables the attacker 
to write a malicious payload called \texttt{clean}
to \texttt{/home/admin/} on disk. %
The attacker then executes the payload
with escalated privileges.
This new attack process (with root privileges) communicates
with the attacker's command-and-control (C\&C) server
at \texttt{161.116.88.72} %
to download and execute
another %
malicious payload
called \texttt{profile}, again with root privileges.
\texttt{profile}, in turn, 
fetches a third payload
called \texttt{xdev} from the C\&C server
and stores the payload in \texttt{/var/log/}. %
\texttt{profile} and \texttt{xdev} lurk in the victim host
to prepare for %
subsequent attacks. 
A few days later, 
the attacker uses \texttt{profile} 
to %
inject malicious code in the \texttt{mail} process
and executes \texttt{mail} with root privileges.
\texttt{mail} then 
performs port scans of all known hosts 
on the victim's network.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=\textwidth, scale=0.5]{figures/scenario_CADET.png}
	\caption{A summary graph that describes attack activity in DARPA's E3-CADETS dataset, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_CADETS}
\end{figure*}

\noindgras{E3-CADETS (\autoref{fig:evaluation:casestudy_CADETS}).}
The attacker (\texttt{81.49.200.166})
connects to
a vulnerable \texttt{Nginx} server
and obtains a shell.
Through the shell,
the attacker successfully downloads a
malicious payload to \texttt{/tmp/vUgefal}
and executes the payload with root privileges.
The elevated process \texttt{vUgefal}
attempts to move laterally to \texttt{154.145.113.18}
and \texttt{61.167.39.128}.
However,
only the attempt at infecting \texttt{61.167.39.128} is successful.
\texttt{vUgefal} further plans to
inject malicious payload to the \texttt{sshd} process.
To do so,
the attacker downloads the payload to \texttt{/var/log/devc},
but the attempted process injection fails.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth, scale=0.5]{figures/scenario_clearscope3.png}
	\caption{A summary graph that describes attack activity in DARPA's E3-ClearScope dataset, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_clearscope3}
\end{figure*}

\noindgras{E3-ClearScope (\autoref{fig:evaluation:casestudy_clearscope3}).}
The attacker exploits
a vulnerability in \texttt{Firefox}
to gain control of a victim host
by browsing \url{www.mit.gov.jo}.
The attacker then loads
the payload \texttt{shared\_files} into
the victim's filesystem
at \texttt{/data/data/org.mozilla.fennec\_firefox\_dev}
and runs it with root privileges.
The attacker's subsequent attempts
to (1) load additional attack modules
and (2) inject the attack payload into a process
fail.
Note that
we were unable to find any
\texttt{execute}- or \texttt{fork}-related behaviors
in the data.
It is unclear whether
ClearScope records them in E3.
Consequently,
malicious activity that leverages
such behaviors is not invisible to \system
(since it is not included in the data to begin with).

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_theia5.png}
	\caption{A summary graph that describes attack activity in DARPA's E5-THEIA dataset, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_theia5}
\end{figure*}

\noindgras{E5-THEIA (\autoref{fig:evaluation:casestudy_theia5}).}
The attacker exploits a vulnerability in \texttt{Firefox}
by browsing \url{www.nhra.com},
connecting the victim host
to C\&C servers (\texttt{189.141.204.211} and \texttt{208.203.20.42}).
The attacker then uses \texttt{/run/shm}
to escalate privileges
and gain access to a list of processes.
The attacker finds
the \texttt{sshd} process
and injects malicious code into the process.
The compromised \texttt{sshd} process
writes to a file \texttt{/var/log/sshdlog}
on the host's filesystem.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_CADET5.png}
	\caption{A summary graph that describes attack activity in DARPA's E5-CADETS dataset, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_CADETS5}
\end{figure*}

\noindgras{E5-CADETS (\autoref{fig:evaluation:casestudy_CADETS5}).}
The attacker sends a malformed \texttt{HTTP POST}
from \texttt{128.55.12.167}
to the victim host
to trigger the \texttt{Nginx}'s backdoor.
The \texttt{HTTP} request \remove{carries }\change{carrying}%
\remove{a magic value }%
\remove{along with} a payload \remove{to }execute\change{s} shell code,
\remove{allowing the attacker's }%
\remove{C\&C server (\texttt{4.21.51.250})}%
\remove{to establish a connection to the victim host.}%
\change{establishing a connection to a C\&C server (\texttt{4.21.51.250}).}
The attacker obtains
\texttt{username} and \texttt{hostname} information
before unexpectedly losing control.
The next day,
the attacker sends the malformed \texttt{HTTP POST} again
and continues the attack
from the C\&C server (\texttt{128.55.12.233}).
The attacker
exfiltrates
the host's environment information
such as \texttt{hostname},
\texttt{passwd},
and \texttt{username},
in the subsequent attack.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_clearscope5.png}
	\caption{A summary graph that describes attack activity in DARPA's E5-ClearScope dataset, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_clearscope5}
\end{figure*}

\noindgras{E5-ClearScope (\autoref{fig:evaluation:casestudy_clearscope5}).}
A user accidentally installs
a malicious \texttt{appstarter} APK \texttt{de.belu.appstarter},
which loads an attack module
called \texttt{busybox}.
\remove{during the installation process.}
This module gives the attacker control from \texttt{77.138.117.150}. \remove{to the victim host.}
The attacker then installs the driver \texttt{msm\_g711tlaw}
into the victim host for privilege escalation.
The attack exfiltrates
\texttt{calllog.db},
\texttt{calendar.db},
and \texttt{mmssms.db}
\remove{with elevated privileges }%
and takes a screenshot.
Two days later,
the attacker exploits \texttt{appstarter} again
to try to
connect to the C\&C server (\texttt{128.55.12.233}) but failed.
\remove{Note that t}\change{T}he ground truth also
describes some malicious activity
of attack payloads called \texttt{lockwatch}
and \texttt{mozilla}.
Upon close inspection,
we discover that the provenance data
related to the malicious activity
is corrupted.
\remove{(\eg a unique node identifier does not refer to}%
\remove{any system entity).}%
We remove the corrupted data
and omit the malicious activity in~\autoref{fig:evaluation:casestudy_clearscope5}.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_optc_day1.png}
	\caption{A summary graph that describes attack activity in DARPA's OpTC dataset in day 1, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_optcday1}
\end{figure*}

\noindgras{OpTC Day 1 (\autoref{fig:evaluation:casestudy_optcday1}).}
The attacker uses a C\&C server (\texttt{132.197.158.98})
to connect to the victim host
and executes a \texttt{powershell} script \texttt{runme.bat}.
The attacker then injects the process \texttt{lsass}
to collect the victim's credential and host information.
The attacker also scans the network
(\eg using \texttt{ping} and \texttt{smb})
and uses \texttt{wmiprvse} to move laterally
to a host at \texttt{142.20.57.147}.
Eventually,
the attacker moves to a host at \texttt{142.20.58.149}
and runs more \texttt{powershell} scripts \texttt{*.ps1}
to collect information. %

\begin{figure*}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_optc_day2.png}
	\caption{A summary graph that describes attack activity in DARPA's OpTC dataset in day 2, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_optcday2}
\end{figure*}

\noindgras{OpTC Day 2 (\autoref{fig:evaluation:casestudy_optcday2}).}
The attacker sends a phishing email
with a payload (\texttt{payroll.docx})
to the victim.
After executing the payload,
the attacker uses the elevated \texttt{powershell}
to performs network scan
and \texttt{wmiprvse} to establish persistence.
The attacker uploads \texttt{plink.exe} to forward port \texttt{3389}
and uses RDP to connect to the host.
Finally, the attacker collects and compresses
host information into \texttt{*.zip}
and runs \texttt{nx.exe} to exfiltrate the files.

\begin{figure*}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/scenario_optc_day3.png}
	\caption{A summary graph that describes attack activity in DARPA's OpTC dataset in day 3, as automatically generated by \system.
		\remove{Colors and dashed elements are added to ease comparison with the ground truth.}}
	\label{fig:evaluation:casestudy_optcday3}
\end{figure*}

\noindgras{OpTC Day 3 (\autoref{fig:evaluation:casestudy_optcday3}).}
\texttt{Notepad++} downloads a malicious
file \texttt{update.exe}, %
which runs an attack payload \texttt{cKfGW.exe}.
The attacker controls \texttt{cKfGW.exe}
through a malicious DNS server (\texttt{53.192.68.50})
to inject system processes
and collect and modify host information.



